Generating Ontologies from Templates: A Rule-Based Approach for Capturing Regularity

We present a second-order language that can be used to succinctly specify ontologies in a consistent and transparent manner. This language is based on ontology templates (OTTR), a framework for capturing recurring patterns of axioms in ontological modelling. The language and our results are independent of any specific DL. We define the language and its semantics, including the case of negation-as-failure, investigate reasoning over ontologies specified using our language, and show results about the decidability of useful reasoning tasks about the language itself. We also state and discuss some open problems that we believe to be of interest.

==> open-problems.tex <==

\section{Open problems}

\subsection{Finite representability}

In general, the semantics for our GBoxes are such that the expansion of a GBox and ontology needs not be finite. To control this, we currently introduce a finite language as a separate concept. This problem, however, raises the following interesting questions:

\begin{itemize}
  \item If $\lang$ is finite, so is $\oexpand^*(G, \ont, \lang)$ for any $G$ and $\ont$. Are
  there other ways to ensure that $\expand(G, \ont, \lang)$ is
  finitely representable, i.e., contains a (finite) ontology?
  \item Given $\lang, G, \ont$, can we decide whether $\expand(G, \ont, \lang)$ is finitely representable?
\end{itemize}

More broadly, the idea behind GBoxes is to capture and represent repeating patterns. To this end, we wish to define a suitable notion of ``nontrivial consequences'' that a a template should capture and that a generator should generate new axioms from. 


\subsection{Entailment problems on KBs represented by Gboxes}

In this paper we showed, among other things, how to compute an expansion given a GBox and an ontology. While doing so clearly allows us to perform standard reasoning tasks on the new ontology, a question of interest is whether and when reasoning on the input ontology and GBox can provide gains in reasoning efficiency. In particular, a GBox-specified ontology can have, if an expansion is computed, many very similar axioms. Reasoning on the generators that produced them directly ought to be more efficient in such cases.

\subsection{Other entailment relations}
So far, we have only considered semantic entailment for generators:
evaluating a template as a query relies on a semantic notion of
querying. This has the obvious benefit of taking ontology reasoning
into account while querying. Consider the ontology $\ont=\{\conc{A}
\sqsubseteq \conc{B}, \conc{B}\sqsubseteq \conc{C}\}$ and the query
$?X\sqsubseteq C$. Then the evaluation of this query over $\ont$ would
include the concepts $\conc{A}$ and $\conc{B}$. However, they would
include a multitude of possibly unwanted, redundant query results, e.g.,
$\{\conc{A}\sqcap \conc{A}, \conc{A}\sqcap \conc{A}\sqcap \conc{A},
\conc{C}, \conc{B}\sqcap \conc{A} \ldots\}$.

Restricting query evaluation to syntactic entailment addresses the
issue of infinite (potentially redundant) results at the cost of
ontology reasoning. In the above example, the syntactic evaluation of
$?X\sqsubseteq \conc{C}$ over $\ont$ is $\{\conc{B}\}$. This is clearly
highly restrictive and likely not always desirable.

Finding suitable entailment relations between these two extremes, ones
that cull the amount of
unwanted, redundant results while retaining the desirable semantic
behavior, would be highly beneficial to GBoxes and is as such an important direction for future work.

\subsection{Stable model semantics}
Current work on GBoxes with negation has focused on semantics where a
unique expansion can be distinguished. For unstratified programs,
however, such restrictions are in general no longer possible. Thus we
would like to adapt a form of stable model semantics to GBoxes to be
able to clearly characterize the possible expansions.





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main-techrep"
%%% End:


==> usecases.tex <==
\section{Outlook}

Another area of future work is motivated by our preliminary analysis
of \emph{logical} ODPs \cite{gangemi2009ontology}.
We found that a number of rather
straightforward, seemingly useful such pattern require some form of
ellipses and/or maximality. Consider, for example, the role closure
pattern on the role $\conc{hasTopping}$: if $\ont$ entails that
$\conc{MyPizza}\sqsubseteq \exists\conc{hasTopping}.X_1\sqcap \ldots
\exists\conc{hasTopping}.X_n$ and $n$ is maximal for pairwise incomparable $X_i$, then
we would like to automatically add  $\conc{MyPizza}\sqsubseteq
\forall\conc{hasTopping}.(X_1\sqcup \ldots \sqcup X_n)$. Additionally,
some ODPs make use of reified entities. The logical ODP for n-ary
relationships is a simple example, where a class is reified.
In such cases, generators may need the capability to create
new entities.
Extending generators to capture some form of ellipses, or unknown number of
variables and maximality conditions on substitutions for variables, or generation
of new entities, will be part of future work. 

For GBoxes to be indeed intention revealing, we will also support
named generators and named sets of axioms in the body or the head of
generators, as in OTTR \cite{OTTR-ISWC18}.   

